Scalable Semi-supervised Learning with Graph-based Kernel Machine

Acquiring labels are often costly, whereas unlabeled data are usually easy to obtain in modern machine learning applications. Semi-supervised learning provides a principled machine learning framework to address such situations, and has been applied successfully in many real-word applications and industries. Nonetheless, most of existing semi-supervised learning methods encounter two serious limitations when applied to modern and large-scale datasets: computational burden and memory usage demand. To this end, we present in this paper the Graph-based semi-supervised Kernel Machine (GKM), a method that leverages the generalization ability of kernel-based method with the geometrical and distributive information formulated through a spectral graph induced from data for semi-supervised learning purpose. Our proposed GKM can be solved directly in the primal form using the Stochastic Gradient Descent method with the ideal convergence rate $O(\frac{1}{T})$. Besides, our formulation is suitable for a wide spectrum of important loss functions in the literature of machine learning (e.g., Hinge, smooth Hinge, Logistic, L1, and {\epsilon}-insensitive) and smoothness functions (i.e., $l_p(t) = |t|^p$ with $p\ge1$). We further show that the well-known Laplacian Support Vector Machine is a special case of our formulation. We validate our proposed method on several benchmark datasets to demonstrate that GKM is appropriate for the large-scale datasets since it is optimal in memory usage and yields superior classification accuracy whilst simultaneously achieving a significant computation speed-up in comparison with the state-of-the-art baselines.

==> GBS3VM_model_vu.tex <==
In this section, we present our proposed \emph{Graph-based Semi-supervised
Kernel Machine} (GKM). We begin with formulating the optimization
problem for GKM, followed by the derivation of an SGD-based solution.
Finally, we present the convergence analysis for our proposed method.
The convergence analysis shows that our proposed method gains the
ideal convergence rate $\text{O}\left(\frac{1}{T}\right)$ for combinations
of the typical loss functions (cf. Section \ref{sec:lossfunc}) and
the smoothness functions with $p\geq1$.

\subsection{GKM Optimization Problem}

Let $\Phi:\mathcal{X}\longrightarrow\mathcal{H}$ be a transformation
from the input space $\mathcal{X}$ to a Reproducing Hilbert Kernel
Space (RHKS) $\mathcal{H}$. To predict label, we use the function
$f\left(\boldsymbol{x}\right)=\transp{\bw}\Phi\left(x\right)-\rho=\sum_{i=1}^{l+u}\alpha_{i}K\left(x_{i},x\right)-\rho$,
where $\bw=\sum_{i=1}^{l+u}\alpha_{i}\Phi\left(x_{i}\right)$ and
$K\left(.,.\right)$ is kernel function. Inspired from the constrained
optimization problem in Eq. (\ref{eq:gen_op2}), the following optimization
problem over graph is proposed
\begin{gather}
\underset{\bw}{\textrm{min}}\,\left(\frac{1}{2}\left\Vert \bw\right\Vert ^{2}+\frac{C}{l}\sum_{i=1}^{l}\xi_{i}+\frac{C'}{|\mathcal{E}|}\sum_{\left(i,j\right)\in\mathcal{E}}\mu_{ij}\left(f_{i}-f_{j}\right)^{2}\right)\label{eq:gb_s3vm_op}\\
\text{s.t.}:\,\forall_{i=1}^{l}:y_{i}\left(\transp{\bw}\Phi\left(x_{i}\right)-\rho\right)\geq1-\xi_{i}\nonumber \\
\forall_{i=1}^{l}:\xi_{i}\geq0\nonumber 
\end{gather}

\noindent where $f_{i}=\transp{\bw}\Phi\left(\boldsymbol{x_{i}}\right)-\rho$.

In the optimization problem in Eq. (\ref{eq:gb_s3vm_op}), we minimize
$\frac{1}{2}\left\Vert \boldsymbol{\bw}\right\Vert ^{2}$ to maximize
the margin to promote the generalization capacity. At the same time,
we minimize $\sum_{\left(i,j\right)\in\mathcal{E}}\mu_{ij}\left(f_{i}-f_{j}\right)^{2}$
to make the prediction function smoother on the spectral graph.

We rewrite the optimization problem in Eq. (\ref{eq:gb_s3vm_op})
in the primal form as follows\footnote{We can eliminate the bias $\rho$ by simply adjusting the kernel.} 

\noindent\begin{equation}
\resizebox{.91\linewidth}{!}{\noindent\begin{minipage}{\linewidth}
\begin{equation*}
\underset{\bw}{\min}\left(\frac{\norm{\bw}^{2}}{2}+\frac{C}{l}\sum_{i=1}^{l}l\left(\bw;z_{i}\right)+\frac{C'}{|\mathcal{E}|}\sum_{\left(i,j\right)\in\mathcal{E}}\mu_{ij}l_{2}\left(\transp{\bw}\boldsymbol{\Phi}_{ij}\right)\right)\end{equation*} \end{minipage} }\label{eq:primal} 
\end{equation}

\noindent where $z_{i}=\left(x_{i},y_{i}\right)$, $l\left(\bw;x,y\right)=\max\left\{ 0,1-y\transp{\bw}\Phi\left(x\right)\right\} $,
$\boldsymbol{\Phi}_{ij}=\Phi\left(x_{i}\right)-\Phi\left(x_{j}\right)$,
$l_{p}\left(t\right)=\vert t\vert^{p}$ with $t\in\mathbb{R}$, and
$p\geq1$.

In the optimization problem in Eq. (\ref{eq:primal}), the minimization
of $\sum_{i=1}^{l}l\left(\bw;x_{i},y_{i}\right)$ encourages the fitness
of GKM on the labeled portion while the minimization of $\sum_{\left(i,j\right)\in\mathcal{E}}\mu_{ij}l_{2}\left(\transp{\bw}\boldsymbol{\Phi}_{ij}\right)$
guarantees the smoothness of GKM on the spectral graph. Naturally,
we can extend the optimization of GKM by replacing the Hinge loss
by any loss function (e.g., Logistic, L1) and $l_{2}\left(.\right)$
by $l_{p}\left(.\right)$ with $p\geq1$. We achieve the following
optimization problem

\noindent\begin{equation}
\resizebox{.91\linewidth}{!}{\noindent\begin{minipage}{\linewidth}\begin{equation*} \underset{\bw}{\min}\left(\frac{1}{2}\norm{\bw}^{2}+\frac{C}{l}\sum_{i=1}^{l}l\left(\bw;z_{i}\right)+\frac{C'}{|\mathcal{E}|}\sum_{\left(i,j\right)\in\mathcal{E}}\mu_{ij}l_{p}\left(\transp{\bw}\boldsymbol{\Phi}_{ij}\right)\right)\end{equation*}\end{minipage} }\label{eq:primal_extend} 
\end{equation}

\noindent where $l\left(\bw;x,y\right)$ is any convex loss function,
and $l_{p}\left(t\right)=\vert t\vert^{p}$ with $p\geq1$.

It is noteworthy that Laplacian Support Vector Machine (LapSVM) \citep{Belkin2006,Melacci2011}
is a special case of GKM using the Hinge loss with the smoothness
function $l_{2}\left(.\right)$.

\subsection{Stochastic Gradient Descent Algorithm for GKM}

We employ the SGD framework proposed in \citep{Lacoste2012} to solve
the optimization problem in Eq. (\ref{eq:primal_extend}) in the primal
form. Let us denote the objective function as
\[
\mathcal{J}\left(\bw\right)\triangleq\frac{\norm{\bw}^{2}}{2}+\frac{C}{l}\sum_{i=1}^{l}l\left(\bw;x_{i},y_{i}\right)+\frac{C'}{|\mathcal{E}|}\sum_{\left(i,j\right)\in\mathcal{E}}\mu_{ij}l_{p}\left(\transp{\bw}\boldsymbol{\Phi}_{ij}\right)
\]

At the iteration $t$, we do the following:
\begin{itemize}
\item Uniformly sample a labeled instance $x_{i_{t}}$ ($1\leq i_{t}\leq l$)
from the labeled portion $X_{l}$ and an edge $\left(u_{t},v_{t}\right)$
from the set of edges $\mathcal{E}$.
\item Define the instantaneous objective function 
\[
\mathcal{J}_{t}\left(\bw\right)=\frac{\norm{\bw}^{2}}{2}+Cl\left(\bw;x_{i_{t}},y_{i_{t}}\right)+C'\mu_{u_{t}v_{t}}l_{p}\left(\transp{\bw}\boldsymbol{\Phi}_{u_{t}v_{t}}\right)
\]
\item Define the stochastic gradient $g_{t}$ 
\begin{align*}
g_{t} & =\nabla_{\bw}\mathcal{J}_{t}\left(\bw_{t}\right)\\
 & =\bw_{t}+C\nabla_{\bw}l\left(\bw_{t};x_{i_{t}},y_{i_{t}}\right)+C'\mu_{u_{t}v_{t}}\nabla_{\bw}l_{p}\left(\transp{\bw_{t}}\boldsymbol{\Phi}_{u_{t}v_{t}}\right)
\end{align*}
where $\nabla_{\bw}l\left(\bw;x,y\right)$ specifies the derivative
or sub-gradient w.r.t to $\bw$.
\item Update $\bw_{t+1}$ with the learning rate $\eta_{t}=\frac{2}{t+1}$
\begin{align*}
\bw_{t+1} & =\bw_{t}-\eta_{t}g_{t}\\
 & =\frac{t-1}{t+1}\bw_{t}-\frac{2C}{t+1}\nabla_{\bw}l\left(\bw_{t};x_{i_{t}},y_{i_{t}}\right)-\frac{2C'\mu_{u_{t}v_{t}}}{t+1}\nabla_{\bw}l_{p}\left(\transp{\bw_{t}}\boldsymbol{\Phi}_{u_{t}v_{t}}\right)
\end{align*}
\item Update $\overline{\bw}_{t+1}$ as follows
\begin{align*}
\overline{\bw}_{t+1} & =\frac{t-1}{t+1}\overline{\bw}_{t}+\frac{2}{t+1}\bw_{t+1}
\end{align*}
\end{itemize}
We note that the derivative $\nabla_{\bw}l_{p}\left(\transp{\bw}\boldsymbol{\Phi}\right)$
w.r.t $\bw$ can be computed as
\[
\nabla_{\bw}l_{p}\left(\transp{\bw}\boldsymbol{\Phi}\right)=p\text{sign}\left(\transp{\bw}\boldsymbol{\Phi}\right)\vert\transp{\bw}\boldsymbol{\Phi}\vert^{p-1}\boldsymbol{\Phi}
\]

\begin{algorithm}[H]
\caption{Algorithm for GKM.\label{alg:gUS3VM}}

\textbf{Input :} $C$, $C'$, $p$ , $K\left(.,.\right)$
\begin{algor}[1]
\item [{{*}}] $\bw_{1}=\bzero$
\item [{{*}}] $\overline{\bw}_{1}=\bzero$
\item [{for}] $t=1$ \textbf{to} $T$
\item [{{*}}] Uniformly sample $i_{t}$ from \{$1,2,...,l$\} and $\left(u_{t},v_{t}\right)$
from the set of edges $\mathcal{E}$
\item [{{*}}] Update $\bw_{t+1}$ 
\begin{align*}
\bw_{t+1}= & \frac{t-1}{t+1}\bw_{t}-\frac{2C}{t+1}\nabla_{\bw}l\left(\bw_{t};x_{i_{t}},y_{i_{t}}\right)-\frac{2C'\mu_{u_{t}v_{t}}}{t+1}\nabla_{\bw}l_{p}\left(\transp{\bw_{t}}\boldsymbol{\Phi}_{u_{t}v_{t}}\right)
\end{align*}
\item [{{*}}] Update $\overline{\bw}_{t+1}$ 
\[
\overline{\bw}_{t+1}=\frac{t-1}{t+1}\overline{\bw}_{t}+\frac{2}{t+1}\bw_{t+1}
\]
\item [{endfor}]~
\end{algor}
\textbf{Output :} $\overline{\bw}_{T+1}$
\end{algorithm}

The pseudocode of GKM is presented in Algorithm \ref{alg:gUS3VM}.
We note that we store $\bw_{t}$ and $\overline{\bw}_{t}$ as $\bw_{t}=\sum_{i}\alpha_{i}\Phi\left(x_{i}\right)$
and $\overline{\bw}_{t}=\sum_{i}\beta_{i}\Phi\left(x_{i}\right)$.
In line 5 of Algorithm \ref{alg:gUS3VM}, the update of $\bw_{t+1}$
involves the coefficients of $\Phi\left(x_{i_{t}}\right)$, $\Phi\left(x_{u_{t}}\right)$,
and $\Phi\left(x_{v_{t}}\right)$. In line 4 of Algorithm \ref{alg:gUS3VM},
we need to sample the edge $\left(u_{t},v_{t}\right)$ from the set
of edges $\mathcal{E}$ and compute the edge weight $\mu_{u_{t}v_{t}}$.
It is noteworthy that in GKM we use the fully connected spectral graph
to maximize the freedom of label propagation and avoid the additional
computation incurred in other kind of spectral graph (e.g., $k$-NN
or $\varepsilon$-NN spectral graph). In addition, the edge weight
$\mu_{u_{t}v_{t}}$ can be computed on the fly when necessary.

\subsection{Convergence Analysis \label{subsec:Convergence-Analysis}}

In what follows, we present the convergence analysis for GKM. In particular,
assuming that the loss function satisfies the condition: $\norm{\nabla_{\bw}l\left(\bw;x,y\right)}\leq A,\,\forall x,y$,
we prove that our GKM achieves the ideal convergence rate $\text{O}\left(\frac{1}{T}\right)$
with $1\leq p<2$ and with $p\geq2$ under some condition of the parameters
(cf. Theorem \ref{thm:regret}). We present the theoretical results
and the rigorous proofs are given in Appendix \ref{sec:Convex-Analysis}.
Without loss of generality, we assume that the feature map $\Phi\left(x\right)$
is bounded in the feature space, i.e., $\norm{\Phi\left(x\right)}=K\left(x,x\right)^{1/2}\leq R,\,\forall x$.
We denote the optimal solution by $\bw^{*}$, i.e., $\bw^{*}=\text{argmin}_{\vectorize w}\,J\left(\bw\right)$.

The following lemma shows the formula for $\overline{\bw}_{t}$ from
its recursive formula.

\begin{lemma}\label{lem:w_t}We have the following statement
\[
\overline{\bw}_{t}=\frac{2}{t\left(t-1\right)}\sum_{i=1}^{t-1}i\bw_{i}
\]

\end{lemma}

Lemma \ref{lem:func} further offers the foundation to establish an
upper bound for $\norm{\bw_{t}}$.

\begin{lemma}\label{lem:func}Let us consider the function $f\left(x;a,b,p\right)=ax^{p-1}-x+b$
where $x\geq0$ and $p\geq1$, $a,\,b>0$. The following statements
are guaranteed

i) If $p<2$ then $f\left(M;a,b,p\right)\leq0$ where $M=\max\left(1,\left(a+b\right)^{\frac{1}{2-p}}\right)$.

ii) If $p=2$ and $a<1$ then $f\left(M;a,b,p\right)\leq0$ where
$M=\frac{b}{1-a}$.

iii) If $p>2$ and $ab^{p-2}\leq\frac{\left(p-2\right)^{p-2}}{\left(p-1\right)^{p-1}}$
then $f\left(M;a,b,p\right)\leq0$ where $M=\left(\frac{1}{\left(p-1\right)a}\right)^{\frac{1}{p-2}}$.

\end{lemma}

Built on the previous lemma, Lemma \ref{lem:wt_norm} establishes
an upper bound on $\norm{\bw_{t}}$ which is used to define the bound
in Lemma \ref{lem:gt}.

\begin{lemma}\label{lem:wt_norm}We have the following statement
\[
\norm{\bw_{t}}\leq M,\,\forall t
\]
where $M$ is defined as 
\[
M=\begin{cases}
\max\left(1,\left(a+b\right)^{\frac{1}{2-p}}\right) & \text{if}\,p<2\\
\frac{b}{1-a} & \text{if}\,p=2,a<1\\
\left(\frac{1}{\left(p-1\right)a}\right)^{\frac{1}{p-2}} & \text{if}\,p>2,ab^{p-2}\leq\frac{\left(p-2\right)^{p-2}}{\left(p-1\right)^{p-1}}
\end{cases}
\]
with $a=C'\left(2R\right)^{p}p$ and $b=CA$.\end{lemma}

Lemma \ref{lem:gt} establishes an upper bound on $\norm{g_{t}}$
which is used in our subsequent theorems.

\begin{lemma}\label{lem:gt}We have the following statement
\[
\norm{g_{t}}\leq G,\,\forall t
\]
where $G=M+CA+C'\left(2R\right)^{p}pM^{p-1}$.\end{lemma}

We now turn to establish the ideal convergence rate $\text{O}\left(\frac{1}{T}\right)$
for our proposed GKM.

\begin{theorem}\label{thm:regret}Considering the running of Algorithm
\ref{alg:gUS3VM}, the following statements hold

i) $\mathbb{E}\left[\mathcal{J}\left(\overline{\bw}_{T+1}\right)\right]-\mathcal{J}\left(\bw^{*}\right)\leq\frac{2G^{2}}{T},\,\forall T$

ii) $\mathbb{E}\left[\norm{\overline{\bw}_{T+1}-\bw^{*}}^{2}\right]\leq\frac{4G^{2}}{T},\,\forall T$ 

\noindent if $1\leq p<2$ or $p=2,\,a<1$ or $p>2,\,ab^{p-2}\leq\frac{\left(p-2\right)^{p-2}}{\left(p-1\right)^{p-1}}$
where $a=C'\left(2R\right)^{p}p$ and $b=CA$.

\end{theorem}

Theorem \ref{thm:regret} states the regret in the form of expectation.
We go further to prove that for all $T\geq T_{0}=\left\lceil \frac{2G^{2}}{\varepsilon\delta}\right\rceil $,
with a high confidence level, $\mathcal{J}\left(\overline{\bw}_{T+1}\right)$
approximates the optimal value $\mathcal{J}\left(\bw^{*}\right)$
within an $\varepsilon$-precision in Theorem \ref{thm:high_prob_J}.

\begin{theorem}\label{thm:high_prob_J}With the probability at least
$1-\delta$, for all $T\geq T_{0}=\left\lceil \frac{2G^{2}}{\varepsilon\delta}\right\rceil $,
$\mathcal{J}\left(\overline{\bw}_{T+1}\right)$ approximates the optimal
value $\mathcal{J}\left(\bw^{*}\right)$ within an $\varepsilon$-precision,
i.e., $\mathcal{J}\left(\overline{\bw}_{T+1}\right)\leq\mathcal{J}\left(\bw^{*}\right)+\varepsilon$
if $1\leq p<2$ or $p=2,\,a<1$ or $p>2,\,ab^{p-2}\leq\frac{\left(p-2\right)^{p-2}}{\left(p-1\right)^{p-1}}$
where $a=C'\left(2R\right)^{p}p$ and $b=CA$.

\end{theorem}


==> lossfunction_vu.tex <==
In this section, we present the suitability of the loss functions
and kernel functions that can be used for GKM. We verify that most
of the well-known loss functions satisfy the necessary condition:
$\norm{\nabla_{\bw}l\left(\bw;x,y\right)}\leq A$ for an appropriate
positive number $A$.
\begin{itemize}
\item \textit{Hinge loss}: 
\begin{align*}
l\left(\bw;x,y\right) & =\max\left\{ 0,1-y\transp{\bw}\Phi\left(x\right)\right\} \\
\nabla_{\bw}l\left(\bw;x,y\right) & =-\mathbb{I}_{\left\{ y\transp{\bw}\Phi\left(x\right)\leq1\right\} }y\Phi\left(x\right)
\end{align*}
Therefore, by choosing $A=R$ we have 
\[
\norm{\nabla_{\bw}l\left(\bw;x,y\right)}\leq\norm{\Phi\left(x\right)}\leq R=A
\]
\item \textit{Smooth Hinge loss}\textbf{ }\citep{Shalev-Shwartz013}:\textbf{
}
\begin{align*}
l\left(\bw;x,y\right) & =\begin{cases}
0 & \text{if}\,\,yo>1\\
1-y\bw^{\top}\Phi\left(x\right)-\frac{\tau}{2} & \text{if}\,\,yo<1-\tau\\
\frac{1}{2\tau}\left(1-yo\right)^{2} & \text{otherwise}
\end{cases}\\
\nabla_{\bw}l\left(\bw;x,y\right) & =-\mathbb{I}_{\left\{ yo<1-\tau\right\} }y\Phi\left(x\right)+\tau^{-1}\mathbb{I}_{1-\tau\leq yo\leq1}\left(yo-1\right)y\Phi\left(x\right)
\end{align*}
where $o=\bw^{\top}\Phi\left(x\right)$.\\
Therefore, by choosing $A=R$ we have
\begin{gather*}
\norm{\nabla_{\bw}l\left(\bw;x,y\right)}=R\left|\tau^{-1}\mathbb{I}_{1-\tau\leq yo\leq1}\left(yo-1\right)\right|+\\
R\mathbb{I}_{\left\{ yo<1-\tau\right\} }\leq\mathbb{I}_{\left\{ yo<1-\tau\right\} }R+\tau^{-1}\tau\mathbb{I}_{1-\tau\leq yo\leq1}R\leq R=A
\end{gather*}
\item \textit{Logistic loss}:
\begin{align*}
l\left(\bw;x,y\right) & =\log\left(1+\exp\left(-y\transp{\bw}\Phi\left(x\right)\right)\right)\\
\nabla_{\bw}l\left(\bw;x,y\right) & =\frac{-y\exp\left(-y\transp{\bw}\Phi\left(x\right)\right)\Phi\left(x\right)}{\exp\left(-y\transp{\bw}\Phi\left(x\right)\right)+1}
\end{align*}
Therefore, by choosing $A=R$ we have
\[
\norm{\nabla_{\bw}l\left(\bw;x,y\right)}<\norm{\Phi\left(x\right)}\leq R=A
\]
\item \textit{L1 loss}:
\begin{align*}
l\left(\bw;x,y\right) & =\vert y-\transp{\bw}\Phi\left(x\right)\vert\\
\nabla_{\bw}l\left(\bw;x,y\right) & =\text{sign}\left(\transp{\bw}\Phi\left(x\right)-y\right)\Phi\left(x\right)
\end{align*}
Therefore, by choosing $A=R$ we have
\[
\norm{\nabla_{\bw}l\left(\bw;x,y\right)}\leq\norm{\Phi\left(x\right)}\leq R=A
\]
\item $\varepsilon$-\textit{insensitive loss}:
\begin{align*}
l\left(\bw;x,y\right) & =\max\left\{ 0,\vert y-\transp{\bw}\Phi\left(x\right)\vert-\varepsilon\right\} \\
\nabla_{\bw}l\left(\bw;x,y\right) & =\mathbb{I}_{\left\{ \vert y-o>\varepsilon\right\} }\text{sign}\left(o-y\right)\Phi\left(x\right)
\end{align*}
where $o=\transp{\bw}\Phi\left(x\right)\vert$.\\
Therefore, by choosing $A=R$ we have
\[
\norm{\nabla_{\bw}l\left(\bw;x,y\right)}\leq\norm{\Phi\left(x\right)}\leq R=A
\]
\end{itemize}
Here $\mathbb{I}_{S}$ is the indicator function which is equal to
$1$ if the statement $S$ is true and $0$ if otherwise.

It can be observed that the positive constant $A$ coincides the radius
$R$ (i.e., $A=R$) for the aforementioned loss functions. To allow
the ability to flexibly control the minimal sphere that encloses all
$\Phi\left(x\right)$(s), we propose to use the squared exponential
kernel function which is given by
\begin{equation}
K\left(x,x'\right)=\sigma_{f}^{2}\text{exp}\left(-\norm{x-x'}^{2}/\left(2\sigma_{l}^{2}\right)\right)\label{eq:kernel}
\end{equation}
where $\sigma_{l}$ is the length-scale parameter and $\sigma_{f}$
is the output variance parameter.

It appears that using the kernel in Eq. (\ref{eq:kernel}) , we have
the following equality
\[
\norm{\Phi\left(x\right)}=K\left(x,x\right)^{1/2}=\sigma_{f}\leq R
\]
Recall that if $p=2$ or $p>2$, Algorithm \ref{alg:gUS3VM} converges
to the optimal solution with the ideal convergence rate $\text{O}\left(\frac{1}{T}\right)$
under specific conditions. In particular, with $p=2$ the corresponding
condition is $a<1$ and with $p>2$ the corresponding condition is
$ab^{p-2}\leq\frac{\left(p-2\right)^{p-2}}{\left(p-1\right)^{p-1}}$
where $a=C'\left(2R\right)^{p}p$ and $b=CA$. Using the squared exponential
kernel function in Eq. (\ref{eq:kernel}), we can adjust the output
variance parameter $\sigma_{f}$ to make the convergent condition
valid. More specifically, we consider two cases:
\begin{itemize}
\item $p=2$: the convergent condition is derived as follows
\begin{align*}
a & <1\goto C'\left(2R\right)^{p}p<1\goto R<0.5\left(pC'\right)^{-1/p}
\end{align*}
We can simply choose $\sigma_{f}$ as 
\begin{align*}
\sigma_{f} & =R=0.5\left(pC'\right)^{-1/p}-\rho=0.5\left(2C'\right)^{-1/2}-\rho
\end{align*}
 where $\rho>0$ is a very small number.
\item $p>2$: the convergent condition is derived as follows
\begin{align*}
ab^{p-2} & \leq\left(p-2\right)^{p-2}\left(p-1\right)^{1-p}\\
C'\left(2R\right)^{p}p\left(CA\right)^{p-2} & \leq\left(p-2\right)^{p-2}\left(p-1\right)^{1-p}\\
C'\left(2R\right)^{p}p\left(CR\right)^{p-2} & \leq\left(p-2\right)^{p-2}\left(p-1\right)^{1-p}\\
R^{2p-2} & \leq\frac{\left(p-2\right)^{p-2}}{2^{p}C^{p-2}C'p\left(p-1\right)^{p-1}}\\
R & \leq\left(\frac{\left(p-2\right)^{p-2}}{2^{p}C^{p-2}C'p\left(p-1\right)^{p-1}}\right)^{\frac{1}{2p-2}}
\end{align*}
We can simply choose $\sigma_{f}$ as 
\[
\sigma_{f}=R=\left(\frac{\left(p-2\right)^{p-2}}{2^{p}C^{p-2}C'p\left(p-1\right)^{p-1}}\right)^{\frac{1}{2p-2}}
\]
\end{itemize}
In case we wish to use the popular radial basic function (RBF) kernel
which is given by 
\[
K\left(x,x'\right)=\text{exp}\left(-\norm{x-x'}^{2}/\left(2\sigma_{l}^{2}\right)\right)
\]
, we can control the second trade-off parameter $C'$ to ensure the
ideal convergence rate $\text{O}\left(\frac{1}{T}\right)$ with $p\geq2$.
More specifically, we also consider two cases:
\begin{itemize}
\item $p=2$: the convergent condition is derived as follows
\begin{align}
a & <1\goto C'<\left(2R\right)^{-p}p^{-1}=0.125\label{eq:p2_RBF}
\end{align}
\item $p>2$: the convergent condition is derived as follows
\begin{align}
ab^{p-2} & \leq\left(p-2\right)^{p-2}\left(p-1\right)^{1-p}\nonumber \\
C'\left(2R\right)^{p}p\left(CA\right)^{p-2} & \leq\left(p-2\right)^{p-2}\left(p-1\right)^{1-p}\nonumber \\
C'\left(2R\right)^{p}p\left(CR\right)^{p-2} & \leq\left(p-2\right)^{p-2}\left(p-1\right)^{1-p}\nonumber \\
C' & \leq\frac{\left(p-2\right)^{p-2}}{2^{p}C^{p-2}p\left(p-1\right)^{p-1}}\label{eq:pgt2_RBF}
\end{align}
\end{itemize}



==> spectral_graph_vu.tex <==

\subsection{Spectral Graph}

Spectral graph is a useful tool to capture the geometrical and distributive
information carried in the data. It is usually formulated as an undirected
graph whose vertices are the data instances. In the context of semi-supervised
learning, we are given a training set $X=X_{l}\cup X_{u}$ where $X_{l}=\left\{ \left(x_{i},y_{i}\right)\right\} _{i=1}^{l}$
is labeled data and $X_{u}=\left\{ x_{i}\right\} _{i=l+1}^{l+u}$
is unlabeled data. We can start with constructing the spectral graph
$\mathcal{G}=\left(\mathcal{V},\mathcal{E}\right)$ where the vertex
set $\mathcal{V}$ includes all labeled and unlabeled instances (i.e.,
$\mathcal{V}=\left\{ x_{i}\right\} _{i=1}^{l+u}$). An edge $e_{ij}=\overline{x_{i}x_{j}}\in\mathcal{E}$
between two vertices $x_{i},\,x_{j}$ represents the similarity of
the two instances. Let $\mu_{ij}$ be the weight associated with edge
$e_{ij}$. The underlying principle is to enforce that if $\mu_{ij}$
is large, then $y_{i}$ and $y_{j}$ are expected to receive the same
label. The set of edges $\mathcal{G}$ and its weighs can be built
using the following ways \citep{Zhu2009}:
\begin{itemize}
\item \textit{Fully connected graph}: every pair of vertices $x_{i}$, $x_{j}$
is connected by an edge. The edge weight decreases when the distance
$\norm{x_{i}-x_{j}}$ increases. The Gaussian kernel weight function
widely used is given by
\[
\mu_{ij}=\text{exp}\left(-\Vert x_{i}-x_{j}\Vert^{2}/\left(2\sigma_{s}^{2}\right)\right)
\]
where $\sigma_{s}$ is known as the bandwidth parameter and controls
how quickly the weight decreases.
\item $k$\textit{-NN}: each vertex $x_{i}$ determines its $k$ nearest
neighbors ($k$-NN) and makes an edge with each of its $k$-NN. The
Gaussian kernel weight function can be used for the edge weight. Empirically,
$k$-NN graphs with small $k$ tend to perform well.
\item $\varepsilon$\textit{-NN}: we connect $x_{i}$ and $x_{j}$ if $\norm{x_{i}-x_{j}}\leq\varepsilon$.
Again the Gaussian kernel weight function can be used to weight the
connected edges. In practice, $\varepsilon$-NN graphs are easier
to construct than $k$-NN graphs.
\end{itemize}
It is noteworthy that when constructing a spectral graph, we avoid
connecting the edge of two labeled instances since we do not need
to propagate the label between them. Figure \ref{fig:sg} illustrates
an example of spectral graph constructed on 3D dataset using $k$-NN
with $k=5$.

\begin{figure}[H]
\begin{centering}
\includegraphics[width=0.8\columnwidth]{SpectralGraph}
\par\end{centering}
\caption{Visualization of a spectral graph on 3D dataset using $k$-NN with
$k=5$.\label{fig:sg}}

\end{figure}


\subsection{Label Propagation}

After building the spectral graph, a semi-supervised learning problem
is formulated as assigning labels to the unlabeled vertices. We need
a mechanism to rationally propagate labels from the labeled vertices
to the unlabeled ones. Again, the key idea here is to encourage $y_{i}$
to have the same label as $y_{j}$ if the weight $\mu_{ij}$ is large. 

To assign labels to the unlabeled instances, it is desirable to learn
a mapping function $f:\,\mathfrak{\mathcal{X}}\longrightarrow\mathcal{Y}$
where $\mathcal{X}$ and $\mathcal{Y}$ are the domains of data and
label, respectively, such that
\begin{itemize}
\item $f\left(x_{i}\right)$ is as closest to its label $y_{i}$ as possible
for all labeled instances $x_{i}\,\left(1\leq i\leq l\right)$.
\item $f$ should be smooth on the whole graph $\mathcal{G}$, i.e., if
$x_{i}$ is very close to $x_{j}$ (i.e., $x_{i}$, $x_{j}$ are very
similar or $\mu_{ij}$ is large), the discrepancy between $f_{i}$
and $f_{j}$ (i.e., $|f_{i}-f_{j}|$) is small.
\end{itemize}
Therefore, we arrive at the following optimization problem \citep{Zhu2009}
\begin{equation}
\underset{f}{\min}\,\left(\infty\times\sum_{i=1}^{l}\left(f_{i}-y_{i}\right)^{2}+\sum_{\left(i,j\right)\in\mathcal{E}}\mu_{ij}\left(f_{i}-f_{j}\right)^{2}\right)\label{eq:gen_op}
\end{equation}

\noindent where by convention we define $\infty\times0=0$ and $f_{i}=f\left(x_{i}\right)$.

The optimization problem in Eq. (\ref{eq:gen_op}) peaks its minimum
as the first term is exactly $0$ and the second term is as smallest
as possible. It can be therefore rewritten as a constrained optimization
problem:
\begin{gather}
\underset{f}{\min}\,\left(\sum_{\left(i,j\right)\in\mathcal{E}}\mu_{ij}\left(f_{i}-f_{j}\right)^{2}\right)\label{eq:gen_op2}\\
\text{s.t.}:\,\forall_{i=1}^{l}:f_{i}=y_{i}\nonumber 
\end{gather}

To extend the representation ability of the prediction function $f$,
we relax the discrete function $f$ to be real-valued. The drawback
of the relaxation is that in the solution, $f(x)$ is now real-valued
and hence does not directly correspond to a label. This can however
be addressed by thresholding $f(x)$ at zero to produce discrete label
predictions, i.e., if $f(x)\geq0$, predict $y=1$, and if $f(x)<0$,
predict $y=-1$.

